Balanced Circle Packings for Planar Graphs

We study balanced circle packings and circle-contact representations for planar graphs, where the ratio of the largest circle's diameter to the smallest circle's diameter is polynomial in the number of circles. We provide a number of positive and negative results for the existence of such balanced configurations.

==> embed-tree.tex <==
% !TEX root = circle-contact.tex
\section{Rectangle-Contact Representation from Embedded Dual}




In this section we show that any contact representation of any maximal outerplanar graph
 $G$ with rectangles gives an embedded orthogonal layout of an augmeneted weak dual
 tree of $G$. We then address the following problem: given a topological orthogonal embedding
 of the augmented dual of $G$, is it possible to transform this layout to a contact representation
 of $G$ with rectangles?






\begin{figure}[htbp]
\centering
\includegraphics[width=0.95\textwidth]{figures/embed-tree.pdf}
\caption
{
(a) An (augmented) outerplanar graph $G$ and its weak dual $T$,
(b)--(c) a contact representation of $G$ with rectangles and
 the corresponding orthogonal layout for $T$,
(d)--(e) a topologically different contact representation of $G$ with rectangles and
 the corresponding orthogonal layout for $T$,
 peripheral regions with 2 corners (f), 3 corners (g), 4 corners (h) and 5 corners (i).
}
\label{fig:embed-tree}
\end{figure}





\newcommand{\tDraw}[1]{\includegraphics[height=1.5ex]{figures/#1.pdf}}


Let $G$ be a maximal outerplanar graph and let $\Gamma$ be a contact representation of $G$
 with rectangles (where no four rectangles touch at a common point); see
 \autoref{fig:embed-tree}(a), (b), (d). We consider an augmented maximal outerplanar graph
 $G'$, where we walk across the outer-cycle of $G$ and for each edge we add a triangular
 face. Construct an orthogonal layout $\Lambda$, which is a subset of $\Gamma$ induced
 by all the points that lie in the boundaries of at least two rectangles. Consider $\Lambda$
 as a drawing of a graph where each point of degree 3 in $\Gamma$ (i.e. internal points on
 common boundaries of three rectangles or external points on common boundaries of two
 rectangles) is a vertex and each segment between pairs of degree-3 points (connected set
 of internal points lying on the common boundaries of exactly two rectangles) is an edge;
 see \autoref{fig:embed-tree}(b)--(c) and \autoref{fig:embed-tree}(d)--(e). Then one can
 see that $\Lambda$ is an orthogonal drawing of the weak dual tree $T$ of $G'$. Call
 $\Lambda$ an orthogonal layout of the weak dual of $G$.


 We augment this layout $\Lambda$ by adding a pair of half-edges at each degree-1 point
 $p$, which gives the information about how the two rectangles incident to $p$ is oriented.
 In particular assume that the segment incident to $p$ is horizontal. Then a {\tDraw{reverseL}}
 (resp. {\tDraw{L}}) implies that the top (resp. bottom) rectangle extends more to the right
 than the bottom (resp. top) rectangle; a {\tDraw{straight}} implies that both the rectangle
 has collinear right sides. Similar intrepretation is implied when the incident segment is vertical.
 Call this augmented layout an extended orthogonal embedding of the weak dual
 of $G$. With extended orthogonal embedding $\Lambda$, there is a topologically unique
 contact representation of $G$ with ractangles that realizes $\Lambda$. 



We now consider the following problem: given an extended orthogonal embedding $\Lambda$
 of the weak dual of a maximal outerplanar graph $G$, is there any contact representation of
 $G$ with rectangles that realizes $Lambda$? Next we give a recognition algorithm for this
 problem. Before we describe this algorithm, we need the following definitions. Given an
 extended orthogonal embedding $\Lambda$ of the weak dual of $G$, consider a
 counterclockwise walk around $\Lambda$: a walk where we alwyas touch $\Lambda$ by our
 left hand. A \textit{peripheral region} is a connected set of segments between two consecutive
 degree-1 points of the orthogonal layout, which starts and ends at a left half-edge and a right
 half-edge, respectively. A \textit{$k$-corners} peripheral region for some positive integer $k$
 is one where the number of times the region turns by a $\Pi/2$ angle is $k$.
\autoref{fig:embed-tree}(f)--(i) illustrate a 2-corner, a 3-corner, a 4-corner and a 5-corner
 peripheral regions, respectively. We now have the following theorem.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{figures/check-layout.pdf}
\caption{Illsutration for the proof of \autoref{th:check-layout}.}
\label{fig:check}
\end{figure}


\begin{theorem}
\label{th:check-layout} Let $\Lambda$ be an extended orthogonal embedding of the weak dual
 of a maximal outerplanar graph $G$. Then $G$ admits a contact representation with rectangles
 that realizes $\Lambda$ if and only if $\Lambda$ has no $k$-corner peripheral region for
 any value of $k>4$.
\end{theorem}
\begin{proof} Assume first that $G$ admits a contact representation $\Gamma$ of $G$ with
 rectangles that realizes $\Lambda$. Then each peripheral region in $\Lambda$ defines a
 rectangle in $\Gamma$. If $\Lambda$ had a $k$-corner peripheral region for some value
 $k>4$, then $\Gamma$ would not be able to realize $\Lambda$ since a rectangle
 has only 4 corners. Thus there is no $k$-corner peripheral region in $\Lambda$ for any $k>4$.

Conversely if all the peripheral regions of $\Lambda$ has at most 4 corners, then we construct
 a contact representation of $G$ with rectangles that realized $\Lambda$ as follows. We
 consider a counterclockwise walk around $\Lambda$ and for each peripheral region $R$ we
 construct a closed region by inserting a poly-arc between two half-edge endpoints of $R$.
 If $R$ is a$k$-corner peripheral region with $k<4$ that we add $4-k$ dummy vertices
 on the poly-arc and consider a $\Pi/2$ turning angle at these vertices. This results in a poly-arc
 closed region for $R$ with exactly four $\Pi/4$ corners. Once we do this for all the peripheral
 region in $\Lambda$, we obtain a ploly-arc layout where each closed region has exactly four
 $\Pi/4$ turning angles (each of this closed region represents a vertex of $G$ uniquely) and
 the summation of angles around each vertex is $2\Pi$. Then due to~\cite{Tam87}, this
 topological layout can be drawn in such a way that each face is a rectangle, which yields our
 desired contact representation of $G$ with rectangles.
 \end{proof}



\subsection{Open Questions}

\begin{enumerate}
	\item Given an extended orthogonal embedding $\Lambda$ of the weak dual of a maximal
	outerplanar graph $G$, is there any contact representation of $G$ with squars that
	realizes $Lambda$? We know that there are some layout (for example a layout where for
	some root vertex $r$, all segments in $\Lambda$ goes to right or down from away from
	$r$) for which there is a square representation. Is it true that for any layout for which there
	is a contact representation with rectangles, there is also a contact representation with
	squares?


	\item Given a maximal outerplanar graph $G$, is there some extended orthogonal
	embedding of the weak dual which can be realized by a balanced contact representation
	of squares?
	
\end{enumerate}




